Concept-Guided LLM Agents for Human-AI Safety Codesign

Generative AI is increasingly important in software engineering, including safety engineering, where its use ensures that software does not cause harm to people. This also leads to high quality requirements for generative AI. Therefore, the simplistic use of Large Language Models (LLMs) alone will not meet these quality demands. It is crucial to develop more advanced and sophisticated approaches that can effectively address the complexities and safety concerns of software systems. Ultimately, humans must understand and take responsibility for the suggestions provided by generative AI to ensure system safety. To this end, we present an efficient, hybrid strategy to leverage LLMs for safety analysis and Human-AI codesign. In particular, we develop a customized LLM agent that uses elements of prompt engineering, heuristic reasoning, and retrieval-augmented generation to solve tasks associated with predefined safety concepts, in interaction with a system model graph. The reasoning is guided by a cascade of micro-decisions that help preserve structured information. We further suggest a graph verbalization which acts as an intermediate representation of the system model to facilitate LLM-graph interactions. Selected pairs of prompts and responses relevant for safety analytics illustrate our method for the use case of a simplified automated driving system.

==> backup/backup.tex <==
\begin{table*}
\centering
\begin{tabular}{|p{1.5cm}|p{5.5cm}|p{10cm}|}
    \hline
    Prompt & Response & Graph \\
    \hline
    What happens if Radar1, Radar2 and GPS have a fault? & 
   {When Radar1, Radar2, and GPS have a fault, the affected components in the system are Radar1, Radar2, GPS, SignalProcessor, PathPlanner, and VehicleController. The fault in these components can have various consequences to the system. For example, the faulty Radar1 and Radar2 can lead to inaccurate detection and tracking of objects, which can affect the overall situational awareness of the system. The faulty GPS can result in incorrect positioning information, which can impact the navigation and guidance capabilities of the system. The faulty SignalProcessor, PathPlanner, and VehicleController can lead to incorrect processing of sensor data, planning of vehicle trajectories, and control of the vehicle, respectively, which can affect the overall performance and safety of the system. It is important to address these faults and ensure proper functioning of the components to maintain the reliability and effectiveness of the system.} & 
    \raisebox{-\totalheight}{\includegraphics[width=0.57\textwidth]{./pics/output_1.png}}\\
    \hline
    Row 2 & Row 2 & \raisebox{-\totalheight}{\includegraphics[width=0.5\textwidth]{./pics/output_2.png}}\\

    \hline
\end{tabular}
\end{table*}


% \begin{itemize}
%     \item Cascading decision tree for LLM to identify right task
%     \item Augmentation with classically calculated fault information
%     \item Phrasing of a natural answer
%     \item system manipulation on IR based on answer
%     \item classical transformation to xml
% \end{itemize}


% \begin{itemize}
%     \item Cascading decision tree for LLM to identify right task
%     \item Augmentation with classically calculated fault information
%     \item Phrasing of a natural answer
%     \item system manipulation on IR based on answer
%     \item classical transformation to xml
% \end{itemize}

==> commands.tex <==


% symbols
\newcommand{\xml}{\textit{xml} }
